The Affiliate Matching Problem: On Labor Markets where Firms are Also Interested in the Placement of Previous Workers

In many labor markets, workers and firms are connected via affiliative relationships. A management consulting firm wishes to both accept the best new workers but also place its current affiliated workers at strong firms. Similarly, a research university wishes to hire strong job market candidates while also placing its own candidates at strong peer universities. We model this affiliate matching problem in a generalization of the classic stable marriage setting by permitting firms to state preferences over not just which workers to whom they are matched, but also to which firms their affiliated workers are matched. Based on results from a human survey, we find that participants (acting as firms) give preference to their own affiliate workers in surprising ways that violate some assumptions of the classical stable marriage problem. This motivates a nuanced discussion of how stability could be defined in affiliate matching problems; we give an example of a marketplace which admits a stable match under one natural definition of stability, and does not for that same marketplace under a different, but still natural, definition. We conclude by setting a research agenda toward the creation of a centralized clearing mechanism in this general setting.

==> Interview Marketplace arxiv/ethics.tex <==


In addition to the ethical questions that are brought about by the above research challenges, we see other important discussion points. Making socially- and morally-laden decisions are necessary steps when designing economic mechanisms; indeed, the allocation of scarce resources, or matching agents to other agents or opportunities, often comes with unavoidable creation of winners and losers.
%
One way to enforce socially desirable outcomes in a matching mechanism is by careful definition and analysis of desiderata, such as stability, of a mechanism. Stability in particular yields one form of fairness---it eliminates justifiable envy---which we as mechanism designers can define in a way to produce outcomes that align with social and moral values of a society. 

Additionally, the way that prestige operates in affiliate marketplaces could potentially be viewed as deleterious---enriching those who are already privileged at the expense of those with fewer means and resources. At issue will be whether a course of study in affiliate matching is about understanding the current practices for the sake of understanding, or if the ultimate goal is reform. If it is the latter, any reform has unintended consequences which could ultimately cause more harm than any intended benefit. We hope that this work serves to contribute in a positive direction towards understanding a current system and its inequities, but we also acknowledge that it might ultimately serve to solidify some of these very ideas. 
